Don't Forget About Pronouns: Removing Gender Bias in Language Models Without Losing Factual Gender Information

The representations in large language models contain multiple types of gender information. We focus on two types of such signals in English texts: factual gender information, which is a grammatical or semantic property, and gender bias, which is the correlation between a word and specific gender. We can disentangle the model's embeddings and identify components encoding both types of information with probing. We aim to diminish the stereotypical bias in the representations while preserving the factual gender signal. Our filtering method shows that it is possible to decrease the bias of gender-neutral profession names without significant deterioration of language modeling capabilities. The findings can be applied to language generation to mitigate reliance on stereotypes while preserving gender agreement in coreferences.

==> sections/X05_ethical_consideration.tex <==
%\todo{recapitalize the ethical considerations.}
We define bias as the connection between a word and the specific gender it is usually associated with. The association usually stems from the imbalanced number of corpora mentions of the word in male and female contexts. This work focuses on the stereotypical bias of nouns  that do not have otherwise denotation of gender (semantic or grammatical). We consider such a denotation as factual gender and want to guard it in the models' representation. 

Our method is applied to language models, hence we recognize potential application in language generation. We envision the case where the language model is applied to complete the text about a person, where we don't have implicit information about their gender. In this scenario, the model should not be compelled by stereotypical bias to assign a specific gender to a person. On the other hand, when the implicit information about a person's gender is provided in the context, the generated text should be consistent.

Language generation is becoming  ubiquitous  in everyday NLP applications (e.g., chat-bots, auto-completion \citet{robert-2020-nlg}). Therefore it is important to ensure that the language models do not propagate sexual discrimination. 

The proposed method can also be implemented in deep models for other tasks, e.g., machine translation systems. In machine translation bias is especially harmful when translating from English to languages that widely denote gender grammatically. In translation to such languages generation of gendered nouns tends to be made based on stereotypical gender roles instead of factual gender information provided in the source language \cite{stanovsky-etal-2019-evaluating}.
